I2V-GS: Infrastructure-to-Vehicle View Transformation with Gaussian Splatting for Autonomous Driving Data Generation

Vast and high-quality data are essential for end-to-end autonomous driving systems. However, current driving data is mainly collected by vehicles, which is expensive and inefficient. A potential solution lies in synthesizing data from real-world images. Recent advancements in 3D reconstruction demonstrate photorealistic novel view synthesis, highlighting the potential of generating driving data from images captured on the road. This paper introduces a novel method, I2V-GS, to transfer the Infrastructure view To the Vehicle view with Gaussian Splatting. Reconstruction from sparse infrastructure viewpoints and rendering under large view transformations is a challenging problem. We adopt the adaptive depth warp to generate dense training views. To further expand the range of views, we employ a cascade strategy to inpaint warped images, which also ensures inpainting content is consistent across views. To further ensure the reliability of the diffusion model, we utilize the cross-view information to perform a confidenceguided optimization. Moreover, we introduce RoadSight, a multi-modality, multi-view dataset from real scenarios in infrastructure views. To our knowledge, I2V-GS is the first framework to generate autonomous driving datasets with infrastructure-vehicle view transformation. Experimental results demonstrate that I2V-GS significantly improves synthesis quality under vehicle view, outperforming StreetGaussian in NTA-Iou, NTL-Iou, and FID by 45.7%, 34.2%, and 14.9%, respectively.

==> 07_supply.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary


\section{More Implement Details}
\textbf{Sequence Selection.} We select 10 sequences captured from the Waymo \cite{sun2020scalability} dataset to conduct experiments. The names of these sequences are listed below:
\begin{itemize}
    \item \texttt{segment-11450298750351730790}
    \item \texttt{segment-12374656037744638388}
    \item \texttt{segment-12820461091157089924}
    \item \texttt{segment-15021599536622641101}
    \item \texttt{segment-16767575238225610271}
    \item \texttt{segment-17612470202990834368}
    \item \texttt{segment-17860546506509760757}
    \item \texttt{segment-2094681306939952000}
    \item \texttt{segment-5372281728627437618}
    \item \texttt{segment-6637600600814023975}
\end{itemize}

\textbf{Baseline Methods.} We compare our method with two sparse view methods and two urban scene reconstruction approaches. (1) DNGaussian \cite{li2024dngaussian} introduces a global-local depth regularized approach for few-shot novel view synthesis. (2) SparseGS \cite{xiong2023sparsegs} proposes softmax-scaling and mode-selection rendering technologies to eliminate artifacts and floaters. (3) StreetGaussian \cite{yan2024street} incorporates time into SH coefficients and utilities 3D bounding boxes to train static and dynamic objectives respectively. (4) $S^3$Gaussian \cite{huang2024textit} proposes a self-supervised method to decompose dynamic and static Gaussians without annotated data.  


\textbf{Derivation of Adaptive Depth Warp.} We first expand the Eq. \ref{eq:forward_Warp} as below:
\begin{equation}
\begin{pmatrix}
x' \\
y' \\
z'
\end{pmatrix}
= KR'R^{-1}K^{-1}
\begin{pmatrix}
x \\
y \\
z
\end{pmatrix}
+ K(T'-R'R^{-1}T)
\label{eq:forward_warp_appendix}
\end{equation}
where $x,y,z$ and $x',y',z'$ are point location in input view $\mathcal{V}_i$ and pseudo view $\mathcal{V}_j'$.

These points can be projected onto image plane with:
\begin{equation}
\frac{1}{||w_{norm}||}
\begin{pmatrix}
u_* \\
v_*\\
1
\end{pmatrix}
= K
\begin{pmatrix}
R & T \\
0 & 1
\end{pmatrix}
\begin{pmatrix}
x_* \\
y_*\\
z_* \\
1
\end{pmatrix}
\label{eq:projection_appendix}
\end{equation}
where $||w_{norm}||$ is used to normalize the homogeneous coordinate and $(u_*, v_*)$ is the pixel coordinate. 

We define $(\Delta u,\Delta v)^T$ as the difference in pixel coordinates for a point in input and pseudo views after projection. Then, expanding Eq. \ref{eq:forward_warp_appendix} and bringing Eq. \ref{eq:projection_appendix} into it, with explicitly expanding $K$, $R$ and $T$ we can as a result obtain:
\begin{equation}
\begin{pmatrix}
\Delta u \\
\Delta v
\end{pmatrix}
=
\frac{1}{z(z + t_z)}
\begin{pmatrix}
f_x t_x z + c_x t_z z - t_z x \\
f_y t_y z + c_y t_z z - t_z y
\end{pmatrix}
\label{eq:warp_pixel_difference_appendix}
\end{equation}

Given an ideal warp distance, where all the pixel differences should not exceed, we can formulate the equation as:
\begin{equation}
\left\| \begin{pmatrix} \Delta u \\ \Delta v \end{pmatrix} \right\|_{\infty} \leq \varepsilon
\label{eq:control_warp_appendix}
\end{equation}

Expanding the Eq. \ref{eq:control_warp_appendix}, we can obtain two inequalities where $\varepsilon,t_x,t_y,t_z, x, y,$ and $z$ are variations. :
\begin{equation}
\begin{cases}
f_xt_x\leq\varepsilon(z_0+t_z)-c_xt_z+\frac{x_0}{z_0}t_z\\
f_yt_y\leq\varepsilon(z_0+t_z)-c_yt_z+\frac{y_0}{z_0}t_z
\end{cases}
\label{eq:warp_inquality_appendix}
\end{equation}

To further simplify the inequalities, we can consider the following situations: 1) $t_z = 0$ and 2) $t_z \neq 0$.
% To ensure the inequalities hold for all pixels, we can consider the following situations: 1) $t_z = 0$ and 2) $t_z \neq 0$.

For $t_z = 0$, we can obtain:
\begin{equation}
\left\{
\begin{aligned}
t_x &\leq \frac{\varepsilon z}{f_x} \\
t_y &\leq \frac{\varepsilon z}{f_y}
\end{aligned}
\right.
\end{equation}
Given $f_x$ and $f_y$ are fixed, $\varepsilon$ is pre-defined, and $z$ is set to the minimum value for a conservative estimate, we can control the relative transformation $t_x$ and $t_y$ to set a proper depth warp. 

For $t_z \neq 0$, we can simplify the Eq. \ref{eq:warp_inquality_appendix} as:
\begin{equation}
\begin{cases}
f_x \frac{t_x}{t_z} \leq \varepsilon - c_x + 2 \sqrt{\frac{\varepsilon x}{t_z}} \\
f_y \frac{t_y}{t_z} \leq \varepsilon - c_y + 2 \sqrt{\frac{\varepsilon y}{t_z}}
\end{cases}
\end{equation}
Since only one variation can be controlled in each inequality, we can set $t_z$ as a fixed value to control $t_x$ and $t_y$ to set a proper depth warp. 

% \textbf{Loss Function.} For input images captured by infrastructures, we optimize Gaussian parameters with:
% \begin{equation}
% \mathcal{L}_{input} = \lambda \cdot \| \hat{I} - I \|_1 + (1-\lambda)  \cdot \text{SSIM}(\hat{I}, I)+  \| \hat{D} - D \|_1 ,
% \end{equation}
% where $\lambda$ is set as 0.8.
% For pseudo views, only the confidence-guided optimization is employed:
% \begin{equation}
%     \mathcal{L}_{pseudo} = \mathcal{L}_{con}.
% \end{equation}
% The overall loss for training is:
% \begin{equation}
%     \mathcal{L} = \mathcal{L}_{input} + \mathcal{L}_{pseudo}.
% \end{equation}

\section{Addition Experiments}
\textbf{Analysis of LiDAR Monocular Depth.} To further evaluate the performance of the proposed LiDAR monocular depth, we compare it with BP-Net \cite{tang2024bilateral}, the SOTA in the depth completion. We present the predicted depth and the LiDAR fitting result that assesses the difference between the predicted depth and LiDAR depth. Fig. \ref{fig:depth_comparison_appendix} shows that our method produces depth maps with clearer object shapes compared to BP-Net. Besides, the fitting result illustrates that our method performs a better alignment with LiDAR depth, highlighting that our predicted depth map is more accurate.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/figures/depth_comparison_appendix.png}
    \caption{The comparison result with BP-Net. The fitting result is used to evaluate the alignment between the predicted depth and LiDAR depth.}
    \label{fig:depth_comparison_appendix}
\end{figure*}


\section{More Results}
Fig. \ref{fig:comparison_result_waymo_appendixl} and Fig. \ref{fig:comparison_result_appendixl} present additional comparative results. We encourage readers to watch the video in the supplementary material for more visualization results.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/figures/more_result_waymo.png}
    \caption{More comparison results on Waymo \cite{sun2020scalability} dataset.}
    \label{fig:comparison_result_waymo_appendixl}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{ICCV2025-Author-Kit/figures/more_result.png}
    \caption{More comparison results.}
    \label{fig:comparison_result_appendixl}
\end{figure*}


